Prompt-and-Rerank: A Method for Zero-Shot and Few-Shot Arbitrary Textual Style Transfer with Small Language Models

We propose a method for arbitrary textual style transfer (TST)--the task of transforming a text into any given style--utilizing general-purpose pre-trained language models. Our method, Prompt-and-Rerank, is based on a mathematical formulation of the TST task, decomposing it into three constituent components: textual similarity, target style strength, and fluency. Specifically, our method first uses zero-shot or few-shot prompting to obtain a set of candidate generations in the target style, and then re-ranks these candidates according to a combination of the three components above. Empirically, our method enables small pre-trained language models to perform on par with state-of-the-art large-scale models while consuming two orders of magnitude less compute and memory. Finally, we conduct a systematic investigation of the effect of model size and prompt design (e.g., prompt paraphrasing and delimiter-pair choice) on style transfer quality across seven diverse textual style transfer datasets.

==> tables-and-figures/fig-cond-prob.tex <==
\begin{figure}[t]
\centering
{\includegraphics[width=0.95\columnwidth]{figures/MainFigure.png}}
\caption{GONE BUT NOT FORGOTTEN (RIP). October 31, 2021 - April 15, 2022. We estimate the conditional $p(x^{(s_2)} | [s_1, x^{(s_1})], s_2)$ as the product of $p(s_2 | x^{(s_2)})$ and $p(x^{(s_2)} | x^{(s_1)})$, where the former term denotes the likelihood of the generated output $x^{(s_2)}$ written in the style $s_2$ and the latter the text-similarity between the input $x^{(s_1)}$ and the output $x^{(s_2)}$.} 
\label{fig:approach}
\end{figure}
